Gaussianizing the Earth: Multidimensional Information Measures for Earth Data Analysis

Information theory is an excellent framework for analyzing Earth system data because it allows us to characterize uncertainty and redundancy, and is universally interpretable. However, accurately estimating information content is challenging because spatio-temporal data is high-dimensional, heterogeneous and has non-linear characteristics. In this paper, we apply multivariate Gaussianization for probability density estimation which is robust to dimensionality, comes with statistical guarantees, and is easy to apply. In addition, this methodology allows us to estimate information-theoretic measures to characterize multivariate densities: information, entropy, total correlation, and mutual information. We demonstrate how information theory measures can be applied in various Earth system data analysis problems. First we show how the method can be used to jointly Gaussianize radar backscattering intensities, synthesize hyperspectral data, and quantify of information content in aerial optical images. We also quantify the information content of several variables describing the soil-vegetation status in agro-ecosystems, and investigate the temporal scales that maximize their shared information under extreme events such as droughts. Finally, we measure the relative information content of space and time dimensions in remote sensing products and model simulations involving long records of key variables such as precipitation, sensible heat and evaporation. Results confirm the validity of the method, for which we anticipate a wide use and adoption. Code and demos of the implemented algorithms and information-theory measures are provided.

==> macros/math_format.tex <==
% Theorems and definitions
\usepackage{amsthm}
% \newtheorem{theorem}{Theorem}
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{corollary}[theorem]{Corollary}
% \newtheorem{definition}{Definition}

\newtheorem{algorithm}{Algorithm}
\usepackage{algpseudocode}

% Counters
\renewcommand{\labelenumi}{{\color{halfgray}(\alph{enumi})}}
\renewcommand{\labelenumii}{\color{halfgray}{\roman{enumii}.}}
\renewcommand{\labelitemi}{{\color{halfgray}-}}%\raisebox{0.3ex}{\tiny$\blacksquare$}}}

\numberwithin{theorem}{chapter}
\numberwithin{definition}{chapter}
\numberwithin{algorithm}{chapter}
\numberwithin{figure}{chapter}

% Maths
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}

\numberwithin{equation}{chapter}
\allowdisplaybreaks

% Shaded boxes


\usepackage{framed}
\newenvironment{remark}[1]{%
  \definecolor{shadecolor}{gray}{0.9}%
  \begin{shaded}{\color{Maroon}\noindent\textsc{#1}}\\%
}{%
  \end{shaded}%
}

% Code snippets
\usepackage{minted}
\definecolor{rulecolor}{rgb}{0.80,0.80,0.80}
\definecolor{bgcolor}{rgb}{1.0,1.0,1.0}
\newminted{python}{bgcolor=bgcolor}

% Todo
\newcommand{\todo}[1]{\textcolor{red}{[TODO] #1}}

% Checkmarks
\usepackage{pifont}% http://ctan.org/pkg/pifont
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

==> macros/notation.tex <==
\newcommand{\A}{\mathbf{A}}
\newcommand{\B}{\mathbf{B}}
\newcommand{\C}{\mathbf{C}}
\newcommand{\D}{\mathbf{D}}

\newcommand{\K}{\mathbf{K}}
\newcommand{\II}{\mathbf{I}}
\newcommand{\KAD}{\K_{\mathrm{AD}}}
\renewcommand{\S}{\mathbf{S}}
\newcommand{\Q}{\mathbf{Q}}

\newcommand{\rota}[1]{\begin{sideways}#1\end{sideways}}

\newcommand{\ip}[2]{\langle {#1},\, {#2} \rangle}
\newcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\nlsum}{\sum\nolimits}

% Definitions.
% --------------------
\newcommand{\Real}{\mathbb R}
\newcommand{\Comp}{\mathbb C}

\def\x{{\mathbf x}}
\def\xk{{\mathbf x}^{(k)}}

\def\A{{\mathbf A}}
\def\B{{\mathbf B}}
\def\C{{\mathbf C}}
\def\LL{\boldsymbol{\Lambda}}
\def\Ak{{\mathbf A}_{(k)}}
\def\Bk{{\mathbf B}_{(k)}}
\def\I{{\mathbf I}}
\def\L{{\cal L}}
\def\U{{\mathbf U}}

\newcommand{\w}{{\mathbf w}}
\newcommand{\W}{{\mathbf W}}
\newcommand{\Z}{{\mathbf Z}}
\newcommand{\V}{{\mathbf V}}
\newcommand{\bb}{{\mathbf b}}
\newcommand{\e}{{\mathbf e}}
\newcommand{\uu}{{\mathbf u}}
\newcommand{\vv}{{\mathbf v}}
\newcommand{\bx}{{\mathbf x}}
\newcommand{\bw}{{\mathbf w}}
\newcommand{\bW}{{\mathbf W}}
\newcommand{\bv}{{\mathbf v}}
\newcommand{\bu}{{\mathbf u}}
\newcommand{\PP}{{\mathbf P}}
\newcommand{\Da}{{\mathbf D_a}}
\newcommand{\PHI}{\boldsymbol{\Phi}}
\newcommand{\PHi}{\boldsymbol{\phi}}
% Macros
\newcommand{\vect}[1]{{\boldsymbol{\mathbf{#1}}}} % vector
\newcommand{\mat}[1]{{\boldsymbol{\mathbf{#1}}}} % matrix
\newcommand{\y}{{\vect y}}
\newcommand{\f}{{\vect f}}
\newcommand{\g}{{\vect g}}
\newcommand{\s}{{\vect s}}
\newcommand{\mean}{{\vect \mu}}
\newcommand{\Sig}{{\mat \Sigma}}
\newcommand{\alp}{{\vect \alpha}}
\newcommand{\bet}{{\vect \beta}}
\newcommand{\kfs}{{\vect k}_{*}}
\newcommand{\kgs}{{\vect c}_{*}}
\newcommand{\kfss}{k_{**}}
\newcommand{\kgss}{c_{**}}
\newcommand{\bethat}{\overline{\vect \beta}}
\newcommand{\Kf}{{\mat K}_\vect{ff}}
\newcommand{\Kg}{{\mat K}_\vect{gg}}
\newcommand{\Kgu}{{\mat C}_{fv}}
\newcommand{\Ku}{{\mat C}_{vv}}
\newcommand{\Lam}{{\mat \Lambda}}
\newcommand{\Lamhat}{\overline{\mat \Lambda}}
\newcommand{\X}{{\mat X}}
\newcommand{\Y}{{\mat Y}}
\newcommand{\KL}[0]{\text{KL}}
\renewcommand{\d}[0]{\text{d}} 
\newcommand{\hyperf}{{\vect \theta}_k}
\newcommand{\hyperg}{{\vect \theta}_g}
\newcommand{\hyper}{{\vect \theta}}
\newcommand{\pmean}{{\vect \mu}}
\newcommand{\pcov}{{\mat \Sigma}}

\newcommand{\dataset}{{\cal D}}
\newcommand{\F}{{\cal F}}
\newcommand{\fracpartial}[2]{\frac{\partial #1}{\partial  #2}}
\newcommand{\maketilde}{\raisebox{0.4ex}{\tiny $\sim$}}

%------------------ Mine
\newcommand{\bigO}[0]{\mathcal{O}} 
\newcommand{\GP}[0]{\mathcal{GP}} 
\newcommand{\model}[0]{\mathcal{M}} 
%\newcommand{\R}[0]{\mathcal{R}} 
\newcommand{\Normal}[0]{\mathcal{N}} 
\newcommand{\Normnat}[0]{\mathcal{N}_\text{nat}} 
\renewcommand{\d}[0]{\text{d}} % derivative
\newcommand{\rank}[0]{\text{rank}} % trace
\newcommand{\rv}[1]{\ensuremath{\boldsymbol{#1}}} % random variable
\newcommand{\rvv}[1]{\ensuremath{\boldsymbol{{#1}}}} % random vector
\newcommand{\E}[0]{\mathbb{E}} 
\newcommand{\prob}{p}
\newcommand{\cov}[0]{\text{Cov}} 
\newcommand{\cut}[1]{} % cut out a part of the text
\newcommand{\Integer}[0]{\mathbb{Z}}  
\newcommand{\Natural}[0]{\mathbb{N}}  
\newcommand{\vectortwo}[2]{\left[\!\!\begin{array}{l}{#1}\\{#2}\end{array}\!\!\right]}
\newcommand{\vectorthree}[3]{\left[\!\!\begin{array}{l}{#1}\\{#2}\\{#3}\end{array}\!\!\right]}
\newcommand{\matrixfour}[4]{\left[\!\!\begin{array}{ll}  #1 & #2\\ #3 & #4\\ \end{array}\!\!\right]} 
\newcommand{\arrayfour}[4]{\left\{\begin{array}{ll}  #1 & #2\\ #3 & #4\\ \end{array}\right.}
\newcommand{\chol}{\operatorname{chol}}
\newcommand{\rot}{\operatorname{ro180}}
\newcommand{\tr}{\operatorname{trace}}
\newcommand{\erf}{\operatorname{erf}}
\newcommand{\erfc}{\operatorname{erfc}}
\newcommand{\diag}[0]{\operatorname{diag}} 
\newcommand{\blockdiag}[0]{\operatorname{bd}} 
\newcommand{\logit}[0]{\operatorname{logit}} 
\newcommand{\probit}{\operatorname{probit}}

\newcommand{\PSI}{\boldsymbol{\Psi}}
\newcommand{\PSi}{\boldsymbol{\psi}}
\newcommand{\aalpha}{\boldsymbol{\alpha}}
\newcommand{\BETA}{\boldsymbol{\beta}}
\newcommand{\h}{{\mathcal H}}
\newcommand{\HH}{{\mathbf K}}
\def\argmin{\mathop{\rm arg~min}}
\def\argmax{\mathop{\rm arg~max}}
\newcommand{\Intg}{\mathbb Z}
\DeclareMathOperator{\Lchula}{\mathcal{L}}
\DeclareMathOperator{\Rchula}{\mathbb{R}}
\DeclareMathOperator{\Ychula}{\mathcal{Y}}
\DeclareMathOperator{\abs}{abs}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\sinc}{sinc}

%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{definition}{Definition}[section]
%\newtheorem{property}{Property}[section]
%\newtheorem{property}[theorem]{Property}



% -------------------------------------------------------------------------
% CHAPTER 09
% -------------------------------------------------------------------------
%% Macros
\newcommand{\vect}[1]{{\boldsymbol{\mathbf{#1}}}} % vector
\newcommand{\mat}[1]{{\boldsymbol{\mathbf{#1}}}} % matrix
% \newcommand{\y}{{\vect y}}
% \newcommand{\f}{{\vect f}}
% \newcommand{\g}{{\vect g}}
% \newcommand{\mean}{{\vect \mu}}
% \newcommand{\Sig}{{\mat \Sigma}}

\newcommand{\Kf}{{\mat K}_\vect{ff}}
% \newcommand{\Kg}{{\mat K}_\vect{gg}}
% \newcommand{\KL}[0]{\text{KL}}
% \renewcommand{\d}[0]{\text{d}}  % WARNING, ALREADY DEFINED
\newcommand{\dataset}{{\cal D}}

% %%------------------ Mine
\newcommand{\bigO}[0]{\mathcal{O}} 
\newcommand{\GP}[0]{\mathcal{GP}} 
\newcommand{\Normal}[0]{\mathcal{N}} 
\newcommand{\prob}{p}

==> sections/5_results.tex <==

\subsection{Entropy}

\begin{figure}[h]
\begin{center}
\setlength{\tabcolsep}{0pt}
\begin{tabular}{m{45mm}m{45mm}}
H (Root Mosture) & Normalized H (Root Moisture) \\
\includegraphics[width=\linewidth]{figures/prelim/rm_entropy.png} &
\includegraphics[width=\linewidth]{figures/prelim/rm_n_entropy.png} \\
H (LST) & Normalized H (LST) \\
\includegraphics[width=\linewidth]{figures/prelim/lst_entropy.png} &
\includegraphics[width=\linewidth]{figures/prelim/lst_n_entropy.png} \\
\end{tabular}
\caption{Root Moisture and Soil Moisture for different spatial-temporal values. We show the entropy and normalized entropy} \label{fig:spatemp_h}
\vspace{0.15cm}
\end{center}
\end{figure}


\subsection{Correlation Measures}

\begin{figure}[h]
\begin{center}
\setlength{\tabcolsep}{0pt}
\begin{tabular}{m{45mm}m{45mm}}
Mutual Info & (b) Normalized Mutual Info  \\
\includegraphics[width=\linewidth]{figures/prelim/rm_mi.png} &
\includegraphics[width=\linewidth]{figures/prelim/rm_nmi.png} \\
RV Coefficient & (b) CKA  \\
\includegraphics[width=\linewidth]{figures/prelim/rm_rv.png} &
\includegraphics[width=\linewidth]{figures/prelim/rm_cka.png} \\
\end{tabular}
\caption{Spatial-Temporal results for \textbf{Root Moisture}.} \label{fig:test_stat}
\vspace{0.15cm}
\end{center}
\end{figure}

\begin{figure}[h]
\begin{center}
\setlength{\tabcolsep}{0pt}
\begin{tabular}{m{45mm}m{45mm}}
Mutual Info & (b) Normalized Mutual Info  \\
\includegraphics[width=\linewidth]{figures/prelim/models/gpp_mi.png} &
\includegraphics[width=\linewidth]{figures/prelim/models/gpp_nmi.png} \\
RV Coefficient & (b) CKA  \\
\includegraphics[width=\linewidth]{figures/prelim/models/gpp_rv.png} &
\includegraphics[width=\linewidth]{figures/prelim/models/gpp_cka.png} \\
\end{tabular}
\caption{Spatial-Temporal results for \textbf{Gross Primary Productivity}.} \label{fig:test_stat}
\vspace{0.15cm}
\end{center}
\end{figure}

\subsection{Distnace Measures}

\begin{figure}[h]
\begin{center}
\setlength{\tabcolsep}{0pt}
\begin{tabular}{m{45mm}m{45mm}}
Random Forest, RMSE) & Linear Regression, RMSE) \\
\includegraphics[width=\linewidth]{figures/prelim/models/sm_rf_rmse.png} &
\includegraphics[width=\linewidth]{figures/prelim/models/sm_rlr_rmse.png} \\
Variation Information & RV RMSE \\
\includegraphics[width=\linewidth]{figures/prelim/models/sm_vi.png} &
\includegraphics[width=\linewidth]{figures/prelim/models/sm_rv.png} \\
% \includegraphics[width=\linewidth]{figures/prelim/lst_cka.png} 
\\
\end{tabular}
\caption{Soil Moisture for different spatial-temporal relations. } \label{fig:dist_sm}
\vspace{0.15cm}
\end{center}
\end{figure}

\begin{figure}[h]
\begin{center}
\setlength{\tabcolsep}{0pt}
\begin{tabular}{m{45mm}m{45mm}}
Random Forest, RMSE) & Linear Regression, RMSE) \\
\includegraphics[width=\linewidth]{figures/prelim/models/gpp_rf_rmse.png} &
\includegraphics[width=\linewidth]{figures/prelim/models/gpp_rlr_rmse.png} \\
Variation Information & RV RMSE \\
\includegraphics[width=\linewidth]{figures/prelim/models/gpp_vi.png} &
\includegraphics[width=\linewidth]{figures/prelim/models/gpp_rv.png} \\
\\
\end{tabular}
\caption{Gross Primary Productivity for different spatial-temporal relations. } \label{fig:dist_gpp}
\vspace{0.15cm}
\end{center}
\end{figure}
